A Market Mechanism for Trading Flexibility Between Interconnected Electricity Markets

Electricity markets differ in their ability to meet power imbalances in short notice in a controlled fashion. Relatively flexible markets have the ability to ramp up (or down) power flows across interties without compromising their ability to reliably meet internal demand. In this paper, a market mechanism to enable flexibility trading amongst market operators is introduced. In the proposed market mechanism, market operators exchange information regarding optimal terms of trade (nodal prices and flows) along interconnection lines at every trading round. Equipped with this information, each market operator then independently solves its own internal chance-constrained economic dispatch problem and broadcasts the updated optimal terms of trade for flows across markets. We show the proposed decentralized market mechanism for flexibility trading converges to a Nash equilibrium of the intraday market coupling game, i.e. a combination of internal market clearing solutions (one for each participating market) and flows and prices along interconnection lines so that no individual market operator has an incentive to modify its own internal solution and/or the terms of trade along interties. For a specific class of chance constraints, we show that the limiting equilibrium outcome is efficient, i.e. it corresponds to the solution of the single market clearing problem for all participating markets. The proposed market mechanism is illustrated with an application to the three-area IEEE Reliability Test System.

==> texFiles/2_ProbFormul.tex <==
%
%
%
%
{\color{red} CE: Reminder. Fuse this section with the following section. Revise writing to introduce variables as you explain the market types...}
ISOs usually run different markets before delivering electricity to the customers. These markets include DA market, intraday market, balancing market, etc. An ISO uses each market to achieve certain set of goals. The purpose of DA market is to schedule slow ramping energy resources to meet expected demand, the intraday market is to give the ISO enough flexibility to meet the demand under a wide range of scenarios, and the balancing market is to ensure that demand and supply are in balance at the time of delivery. The focus of this paper is on the intraday markets, yet the underlying concept can be applied to the DA market as well as the balancing market. In the next section we briefly detail the intraday market.
%
\subsection{Intraday Market Clearing Model}
Day-ahead (DA) market, intraday market, and balancing markets are three common markets that ISO uses to schedule it resources in order to meet its demand. The DA market is executed one day prior to the actual time of power delivery, while the intraday markets are often executed hours before the power delivery. In clearing these markets, there are uncertainties about the actual realization of the demands and renewable energy productions. This paper focuses on the \textit{intraday market}, and the goal of the ISO is to schedule its available energy resources such that, with a certain confidence level, it would be able to meet the demand of its customers. In this paper, we assume that the ISO uses \textit{chance-constraint optimization} to clear the market. 

In clearing the intraday market, ISO receives bids from generation units, and uses some estimated probabilistic profile to model the uncertain demand and renewable power generation. The ISO also inputs the commitments of the power generation units in the DA market and the future/forward markets. In the following section we detail the chance-constraint formulation for the proposed decoupled intraday economic dispatch problem.

==> texFiles/4_BlackBox.tex <==
%
%
%
%\blue{CE: I suggest we first describe the decentralized problem (the problem we  solve) and then give the benchmark. The way it is, it is not clear what (2-8) is a benchmark for. }
%
%In this section we address the fundamental question we face when designing coupling markets: \textit{What is the best outcome that we can get from any coupling market mechanism?} To answer this question, we need to be specific about the term \textit{best}. In the context of market mechanism design, the \textit{best} market outcome is the market outcome with highest social welfare, or equivalently, with lowest total cost of generation. We refer to this optimal market outcome as \textit{social optimum}, and solve the \textit{social optimization problem} to find it.

%To formulate the social optimization problem we consider a hypothetical case where there is an omniscient ISO that knows the cost functions of the generators and the nodal demands of all regions. 
% the private information of the regions and clears the chance-constraint intraday market. We are interested in the dispatched of the generators as well as power exchanges and the rates over the tie-lines.
%For simplicity, in this paper we consider DC power networks. The chance-constraint market clearing model for the intraday market is in the following:
%
%\begin{flalign}
%    & \min V = \sum_{a \in \mc{A}} \sum_{g \in \mc{G}_a} C_{a,g} (q_{a,g})  \label{eq::cen_obj_fun}  \\
%    & \mbox{s.t.}    \nn \\
%    & \mathbf{B}_{a} \bm{\theta}_{a} + \mathbf{R}_{a} \mathbf{T}_{a} \preceq \mathbf{M}_{a} \mathbf{Q}_{a} + \mathbf{P}_{a} - \bm{u}_{a}, \hspace{4pt} (\bm{\alpha}_{a}), \hspace{7pt} \forall a \in \mc{A}, \label{eq::cen_load_bal_0}
%\end{flalign}
%\begin{flalign}
%    & \underline{\mathbf{Q}}_a \leq \mathbf{Q}_a \leq \overline{\mathbf{Q}}_a, \hspace{65pt} (\nu_{a,g} , \lambda_{a,g}), \hspace{7pt} \forall a \in \mc{A},
%\end{flalign}
%\begin{flalign}
%    & - \overline{H}_{a,(i,j)} \leq \frac{\theta_{a,i} - \theta_{a,j}}{x_{a,(i,j)}} \leq \overline{H}_{a,(i,j)}, \hspace{6pt} (\kappa_{a,(i,j)}, \eta_{a,(i,j)}), \nn \\
%    & \hspace{130pt} \forall (i,j) \in \mc{H}_a, \hspace{7pt}  \forall a \in \mc{A},
%\end{flalign}
%\begin{flalign}
%    & T_{a,(i,j)} = \frac{\theta_{a,i} - \theta_{a',j}}{\bar{x}_{a,(i,j)}}, \hspace{10pt} (\xi_{a,(i,j)}), \nn \\
%    & \hspace{133pt} \forall (i,j) \in \mc{T}_a, \hspace{7pt} \forall a \in \mc{A},
%\end{flalign}
%\begin{flalign}
%    & -\overline{T}_{a,(i,j)} \leq T_{a,(i,j)} \leq \overline{T}_{a,(i,j)}, \hspace{10pt} (\bar{\kappa}_{a,(i,j)}, \bar{\eta}_{a,(i,j)}), \nn \\
%    & \hspace{133pt} \forall (i,j) \in \mc{T}_a, \hspace{7pt} \forall a \in \mc{A}, \label{eq::TcenMarkIneq}
%\end{flalign}
%\begin{flalign}
%    & \sum_{g \in \mc{G}_a} q_{a,g} + \mathbf{1}^{\top} \mathbf{P}_a - \hspace{-4pt} \sum_{(i,j) \in \mc{T}_a} T_{a,(i,j)} \geq \mc{F}_{L_a}^{-1} \left( 1 - t_a \right), \nn \\
%    & \hspace{164pt} (\gamma_a), \hspace{7pt} \forall a \in \mc{A}, \label{eq::cen_load_bal_5} \\
%    & \theta_{1,1} = 0,   \label{eq::cen_theta_1}
%\end{flalign}
%
%where $\mc{A}$ is a set of areas, $q_{g,a}$ and $C_{a,g}$ are power output and a strictly convex cost function of generator $g$ in area $a$. $\mathbf{B}_a$ is the admittance matrix of area $a$, $\mathbf{P}_a$ is the vector of aggregated forward and DA schedules of generators at nodes in area $a$. $\mc{G}_a$ is a set of generators participating in the intraday market in region $a$, and $\mathbf{Q}_a$ is a vector of their power generations. The matrix $\mathbf{M}_a$ maps the generating units in $\mc{G}_a$ to buses in region $a$. The vector $\bm{u}_a$ denotes point forecasts of the nodal demands in region $a$. $\underline{\mathbf{Q}}_a$ and  $\overline{\mathbf{Q}}_a$ are vectors of lower bound and upper bound power limits of the generators in $\mc{G}_a$. $\mc{H}_a$ is a set of transmission lines in region $a$. $ \overline{H}_{a,(i,j)}$ and $x_{a,(i,j)}$ are the line capacity of the transmission line between nodes $i$ and $j$ in region $a$, and its reactance. $\mc{T}_a$ is a set of tie-lines connected to area $a$; and $T_{a,(i,j)}$, $\overline{T}_{a,(i,j)}$ and $\bar{x}_{a,(i,j)}$ are the flow on the tie-line between node $i$ in region $a$ and node $j$ in a neighboring area, its capacity, and its reactance respectively. $\mathbf{T}_a$ is a vector of flows of the tie-lines connected to area $a$; and $\mathbf{R}_a$ is the incidence matrix mapping tie-line power flow to the nodes in area $a$. The total demand in region $a$ is modeled as a random variable $L_a$, and $\mc{F}_{L_a} (\cdot)$ is its cumulative probability distribution function. $1-t_a$ is the confidence level required for area $a$. Variables is parenthesis after a constraint represent corresponding dual variables.

%The objective function is the total cost of generation across all regions. Constraint \eqref{eq::cen_load_bal_0} has an interesting interpretation. Note that at the time of intraday market there is still some uncertainty about the demand. The goal of the ISO is two-fold:
%\begin{itemize}
%    \item first, to be able to meet the forecast demand of each node (cf. \eqref{eq::cen_load_bal_0}), and
%    \item second, to guarantee that, at least with certain confidence level, the total power generation of each region is sufficient to cover its total demand (cf. \eqref{eq::cen_load_bal_5}),
%\end{itemize} 
%all with the lowest total cost of generation. Hence, in the formulation we do not enforce strict load balance on the nodes (cf. \eqref{eq::cen_load_bal_0}).

%If we solve the centralized optimal power flow (OPF) problem, \eqref{eq::cen_obj_fun} - \eqref{eq::cen_load_bal_5}, we get the \textit{social optimum} solution: $\{ \mathbf{Q}_{a}^{\ast}, \mathbf{T}_{a}^{\ast}, \bm{\theta}_{a}^{\ast}\}, \hspace{5pt} \forall a \in \mc{A}$. We use the superscript " $\ast$ " to indicate primal and dual variables at social optimum solution.

%The goal of coupling mechanism is to design a set of markets that operate on each region and are coupled through some information exchange along tie-lines, such that the market outcome of these coupled markets would be the same as the \textit{social optimum} solution.


%\subsection{Intraday Market Clearing as Black-box Optimization}

We will model market clearing by independent market operators as the solution of a {\em black-box} convex optimization problem. Let $\mathcal{A}=\{1,\dots,A\}$ denote the index set of different markets. 
Intraday clearing for market $a \in \mathcal{A}$ aims to identify adjustments to power generation $\Delta P_{a,g}$ (for all generators $g$ located in market $a$) and interconnection flows $\Delta T_{a,(i,j)}$ (for all interconnection lines $(i,j)$) so as to minimize a given objective $V_a$ while meeting reliability constraints.

We will use a DC approximation to power flow, i.e. the resulting flow along intertie $(i,j)$ must satisfy: 
\begin{equation}
T_{a,(i,j)}+\Delta T_{a,(i,j)}
=\frac{\theta_{a,i} - \theta_{a',j}}{\bar{x}_{a,(i,j)}}
\label{DC_flow}
\end{equation}
where $T_{a,(i,j)}$ is the scheduled flow, $\theta_{a,i}$ and $\theta_{a',j}$ are respectively, the angles at node $i$ and node $j$ (ends of the line) and $\bar{x}_{a,(i,j)}$ is the line's reactance.

The {\em external} input parameters for clearing market $a$ are {\em (i)} the terms of trade quoted by adjacent markets $a' \in \mathcal{A}\backslash{a}$ in the form of the willingness to pay for adjustments in interconnection flows (i.e. flexibility) $\delta_{a',(i,j)}$, the capacity prices (per unit flow) for interconnection lines, say $\mu_{(i,j)}$ (which we denote in vector notation as $(\bm{\delta}_{-a},\bm{\mu})$) and {\em (ii)} the angles at the corresponding ends of the interconnection lines $\theta_{a',j}$ (which we denote in vector notation as $\bm{\theta}_{-a}$). We emphasize that $\bm{\theta}_{-a}$ contains the angle of only those nodes that are one end of the tie-lines connecting to market $a$.


The problem that the market operator of region $a \in \mathcal{A}$ solves in the intraday market can be generically stated as the following {\em black-box} convex optimization problem:
\begin{align}
    & \min_{\bm{\Delta} \mathbf{P}_a,\bm{\Delta} \mathbf{T}_a, \bm{\theta}_{a}} V_a(
   \bm{\Delta} \mathbf{P}_a,\bm{\Delta} \mathbf{T}_a, \bm{\theta}_{a}; \bm{\delta}_{-a},\bm{\mu} ) \label{eq::generObjFun} \\
  & \mbox{s.t.}   \nn \\
  & \mbox{Demand - supply constraints} \\
    & \mbox{Line-flow Constraints for within-region lines} \\
    & \mbox{Line-flow Constraints for tie-lines} ~~~(\bm{\theta}_{-a})
    \label{eq::generTielineCons} \\
    & \mbox{Other reliability constraints} \label{eq::generRelibCons}
\end{align}

where $V_a$ is a strictly convex objective function of $(\bm{\Delta} \mathbf{P}_a, \bm{\Delta} \mathbf{T}_a, \bm{\theta}_{a})$, i.e. the updates in the schedules of the generators and the transmission flows, and the nodal angles respectively. Constraints (2)-(6) defined the set of feasible intraday market adjustments which we shall denote by $\mathcal{F}_a(\bm{\theta}_{-a})$.

We shall denote by $(\widehat{\bm{\Delta}\mathbf{P}}_a, \widehat{\bm{\Delta} \mathbf{T}}_a, \widehat{\bm{\theta}}_{a}) \in \mathcal{F}_a(\bm{\theta}_{-a})$ the solution to the black-box problem (1)-(5) and $\widehat{\bm{\delta}}_{a}$ is the vector of shadow prices associated to flow on the tie-lines.

This general model encompasses a wide variety of market clearing choices. For example, one market might use a chance constrained formulation (as is discussed in section \ref{5_ChanceConsForm} below) while another market might use robust optimization or scenario-based stochastic programming. 

%{\color{darkgreen}
%The vector $\bm{\delta}_a$ can be considered as the bids that market operator $a$ submits to the neighboring regions for importing/exporting flexibility from/to them. The optimality conditions indicate that $\bm{\delta}_a$ should be a function of the dual variables associated with the flexibility trades on the tie-lines. Hence, $\widehat{\bm{\delta}}_{a}$ is the \textit{calculated} $\bm{\delta}_a$ based on the dual variables of \eqref{eq::generObjFun}-\eqref{eq::generRelibCons}.
%The exact form of such function depends on the exact form of such function depends on the exact formulation that the intra-day market formulation that the market operator uses. Hence we use the notation $\widehat{\bm{\delta}}_{a}$ to emphasize that the willingness to pay is derived from the solution of \eqref{eq::generObjFun}-\eqref{eq::generRelibCons}.
%}
%{\color{red} Hossein: I do not understand the previous paragraph.}

%{\color{purple} I tried to explain the sentence: "and $\widehat{\bm{\delta}}_{a}$ is the vector of shadow prices associated to flow on the tie-lines"; and the fact that unlike $\mu$ or $\theta$, there is no formula given for the $\delta$, and the reason is that \textbf{$\bm{\delta}_{a}$ does not appear in} \eqref{eq::generObjFun}-\eqref{eq::generRelibCons} for region $a$, but shows up in the other regions formulations. However, we know that market operator tries to behave optimally, leading to the fact that $\delta$ would eventually be a function of dual variables of the \eqref{eq::generObjFun}-\eqref{eq::generRelibCons}.}



%
%

